Channel Modeling for FR3 Upper Mid-band via Generative Adversarial Networks

The upper mid-band (FR3) has been recently attracting interest for new generation of mobile networks, as it provides a promising balance between spectrum availability and coverage, which are inherent limitations of the sub 6GHz and millimeter wave bands, respectively. In order to efficiently design and optimize the network, channel modeling plays a key role since FR3 systems are expected to operate at multiple frequency bands. Data-driven methods, especially generative adversarial networks (GANs), can capture the intricate relationships among data samples, and provide an appropriate tool for FR3 channel modeling. In this work, we present the architecture, link state model, and path generative network of GAN-based FR3 channel modeling. The comparison of our model greatly matches the ray-tracing simulated data.

==> abstract.tex <==

% Modern cellular systems
% rely increasingly on simultaneous communication in multiple discontinuous bands
% for macro-diversity and increased bandwidth.  
% Multi-frequency communication is particularly crucial in the
% millimeter wave (mmWave) and Terahertz (THz) frequencies,
% as these bands are often coupled with lower frequencies
% for robustness.
% Evaluation of these systems
% requires statistical models that can capture the joint distribution of the channel paths across multiple frequencies.  
% This paper presents a general neural network based methodology for training multi-frequency double directional statistical channel models.  
% In the proposed approach, each is described as a multi-clustered set, and a generative adversarial network (GAN) is trained to generate random multi-cluster profiles where the generated cluster data includes the angles and delay of the clusters along with the vectors of random received powers, angular, and delay spread at different frequencies.  
% The model can be readily applied for multi-frequency link or network layer simulation.  
% The methodology is demonstrated on modeling urban micro-cellular links at \SI{28}{} and \SI{140}{GHz} trained from extensive ray tracing data.
% The methodology makes
% minimal statistical assumptions and experiments show the model can capture
% interesting statistical relationships between frequencies.

